Entanglement, Renormalization and Effective Field Theories

We develop the idea that renormalization, decoupling of heavy particle effects from low energy physics and the construction of effective field theories are intimately linked to the momentum space entanglement of disparate modes of an interacting quantum field theory. Using unitary transformations to decouple these modes at the perturbative level, we show in a scalar field theoretical model with light and heavy fields, how renormalization may be consistently implemented and how the low energy effective field theory can be constructed. We also obtain a renormalization group equation in this framework and apply it to the scalar field theoretical model.

==> Calculation/Calculation.tex <==

\section{Decoupling and Renormalization of A Scalar Field Theory}
\label{sec:Calc}
In this chapter we will work in the weak coupling regime of a scalar field theory with both heavy and light fields. Because we will be discussing renormalization in the Hamiltonian framework, we will consider mode expansions at a fixed time or effectively, we will be working in the Schrodinger picture.
\subsection{Preliminaries}
\label{subsec:ch31}
Our subsequent analysis will apply to a scalar field theory with heavy and light fields ($\Phi_H$ and $\Phi_L$ respectively) with dynamics given by the following Hamiltonian:\\
\begin{equation}
\label{eq:x}
    \begin{aligned} H=& \int d^{3} x \left(\frac{1}{2}\left((\partial \Phi_{L})^{2}+m^{2}\Phi_{L}^{2}\right)+\frac{1}{2}\left((\partial \Phi_{H})^{2}+M^{2}\Phi_{H}^{2}\right)\right.\\
    &\left.+\frac{\lambda_{0}}{4 !} \Phi_{L}(x)^{4}+\frac{\lambda_{1}}{2} \Phi_{H}(x) \Phi_{L}(x)^{2}+\frac{\lambda_{2}}{4} \Phi_{L}(x)^{2} \Phi_{H}(x)^{2}+\frac{\lambda_{3}}{4 !} \Phi_{H}(x)^{4} 
    \right).
    \end{aligned}
\end{equation}
\indent The fields have the usual mode expansions, however, we will need to consider light fields carefully. This is because the light fields contain two parts, one is the low frequency mode $\phi(x)$ and the other is the high frequency mode $\chi (x)$. In order to correctly project onto the low energy subspace, we want only low frequency fields $\phi(x)$ to appear in external lines. This can be taken into account in the usual expansion of all the fields (in Schrodinger picture) in the following manner:\\
\begin{subequations}\label{eq:y}
\begin{align}
\label{eq:y:1}
\phi(x)=\sum_{p<M} \frac{1}{\sqrt{2V \epsilon_{p}}}\left(b_{p} e^{i \boldsymbol p \boldsymbol x} +b_{p}^{\dagger} e^{-i \boldsymbol p \boldsymbol x}\right),
\\
\label{eq:y:2}
\chi(x)=\sum_{M<p} \frac{1}{\sqrt{2V \epsilon_{p}}}\left(b_{p} e^{i \boldsymbol p \boldsymbol x} +b_{p}^{\dagger} e^{-i \boldsymbol p \boldsymbol x}\right),
\\
\label{eq:4:3}
\Phi_{L}(x)=\sum_{p} \frac{1}{\sqrt{2V \epsilon_{p}}}\left(b_{p} e^{i \boldsymbol p \boldsymbol x} +b_{p}^{\dagger} e^{-i \boldsymbol p \boldsymbol x}\right),
\\
\label{eq:y:4}
\Phi_{H}(x)=\sum_{k} \frac{1}{\sqrt{2V \omega_{k}}}\left(a_{k} e^{i \boldsymbol k \boldsymbol x} +a_{k}^{\dagger} e^{-i \boldsymbol k \boldsymbol x}\right).
\end{align}
\end{subequations}

From the expansion, we see that the $\phi$ and the $\chi$ fields are orthogonal, i.e., $\int d^{3}x\, \phi(x) \chi(x)=0$. In the following we will not use the mode expansion of $\phi(x)$ .\\
\indent As discussed earlier, we want to split the total Hamiltonian into four parts: $H_{1}$ only contains low frequency modes of light particles; $H_{2}$ contains both the free part of heavy particles and high frequency modes of light particles; $H_{A}$ contains only creation or annihilation operators, for example terms like $aab$, $a^{\dagger}a^{\dagger}b^{\dagger}$, etc; and $H_{B}$ contains combinations of creation and annihilation operators, for example terms like, $b^{\dagger}a\phi(x)$ and $a^{\dagger}abb$, etc. Thus,
\begin{align}
H = H_1 + H_2 + H_A + H_B.
\end{align}
For our case,
\begin{subequations}\label{eq:y}
\begin{align}
\label{eq:y:1}
H_{1}&=\int d^{3} x \left(
    \frac{1}{2}\left((\partial \phi)^{2}+m^{2}\phi^{2}\right)+\frac{\lambda_{0}}{4 !} \phi^{4}(x)\right),\\
\label{eq:y:2}
H_{2}&=\int d^{3} x \sum_{k} \omega_{k}a_{k}^{\dagger}a_{k}+\sum_{M<p}\epsilon_{p}b_{p}b_{p}^{\dagger}.
\end{align}
\end{subequations}
However, $H_{A}$ and $H_{B}$ are rather involved and will not be explicitly displayed here. As we proceed with the calculation, we will simply pick out the relevant terms in these by analyzing the coupling coefficient and the number of low energy light particles.  \\
\indent We argued earlier that $H_{decoupled}=\bra{0_{high}} \omega^{\dagger} H \omega \ket{0_{high}}$, where $\omega$ denotes a series of unitary transformations, $\omega=\omega_{0} \omega_{1} \dots \omega_{n} \dots$. Our calculations will be limited to the first loop order and for these, we only need the first two terms in the unitary transformations:\\
\begin{equation}\label{eq:x}
    \begin{aligned} \omega^{\dagger} H \omega = e^{-i \Omega_{1}} e^{-i \Omega_{0}}\left(H_{1}+H_{2}+H_{A}+H_{B}\right) e^{i \Omega_{0}} e^{i \Omega_{1}}
    \end{aligned}
\end{equation}
\indent The right hand side of the above simplifies to\\ 
\begin{equation}\label{eq:x}
    \begin{aligned} &H_{1}+H_{2}+H_{B}+\frac{i}{2}[H_{A},\Omega_{0}]+i[H_{B},\Omega_{0}]-\frac{1}{3}[[H_{A},\Omega_{0}],\Omega_{0}]\\
    &-\frac{1}{2}[[H_{B},\Omega_{0}],\Omega_{0}]-\frac{1}{2}[[H_{1},\Omega_{0}],\Omega_{0}]+i[H_{B},\Omega_{1}]+O(\frac{1}{M})
    \end{aligned}
\end{equation}
In deriving the above we have set the cut-off energy scale to the heavy mass M and used the condition that the unitary transformations do not take us out of the high energy vacuum, i.e., $i\left[H_{2}, \Omega_{0}\right] + H_{A} = 0$, $i\left[H_{1}, \Omega_{0}\right] + i\left[H_{2}, \Omega_{1}\right] = 0$.

In the next two sections we will study decoupling and renormalization in this scalar field theory by calculating the decoupled Hamiltonian up to order $ O(\frac{1}{M^{2}})$ at one loop level for the two and four point functions. The calculational techniques are far removed from the usual Feynman diagram methods, however, we have noticed that the Feynman diagrams provide a very good indication of which term in the expansion, eq.(3.6) contribute to the process of interest. Thus in the following, even though we are not using the usual Feynman-Dyson perturbative expansion, we will still refer to the corresponding diagrams in guiding us as to the choice of the relevant terms in eq.(3.6).
\subsection{Decoupling}
\label{subsec:ch32}
\subsubsection{Two Point Function Calculation}
\label{subsubsec:ch321}
\begin{figure}[tbp]
\centering 
\subfigure[]{\includegraphics[width=.25\textwidth]{Figures/A.png}\label{fig:ch31a}}
\hfill
\subfigure[]{\includegraphics[width=.25\textwidth]{Figures/D.png}\label{fig:ch31d}}
\hfill
\subfigure[]{\includegraphics[width=.2\textwidth]{Figures/C.png}\label{fig:ch31c}}
\hfill
\subfigure[]{\includegraphics[width=.25\textwidth]{Figures/B.png}\label{fig:ch31b}}
\caption{\label{fig:i} One loop two point functions. Dashed lines represent heavy fields and solid lines represent light fields.}
\end{figure}
There are four contributions to the two point function at one loop order which we choose to specify through ordinary Feynman diagrams. Consider the Figure \ref{fig:ch31a} diagram which comes from the $\frac{\lambda_{0}}{4!}\Phi_{L}(x)^{4}$ term in the total Hamiltonian and make the mode expansion for the $\phi^{2}\chi^{2}$ piece:
\begin{equation}\label{eq:x}
    \begin{aligned} 6\frac{\lambda_{0}}{4 !} \int d^{3}x\, \sum_{M<k}\sum_{M<p} \frac{1}{\sqrt{2V\epsilon_{k}}}\frac{1}{\sqrt{2V\epsilon_{p}}} e^{i\left(\boldsymbol k - \boldsymbol p \right) \boldsymbol x} b_{k}b_{p}^{\dagger} \phi^{2}(x).
    \end{aligned}
\end{equation}
Normal ordering this term gives\\
\begin{equation}\label{eq:x}
    \begin{aligned} 6\frac{\lambda_{0}}{4 !} \int d^{3}x\, \sum_{M<k}\sum_{M<p} \frac{1}{\sqrt{2V\epsilon_{k}}}\frac{1}{\sqrt{2V\epsilon_{p}}} e^{i\left(\boldsymbol k - \boldsymbol p \right) \boldsymbol x} \left(\left[b_{k},b_{p}^{\dagger} \right]+b_{p}^{\dagger}b_{k}\right) \phi^{2}(x),
    \end{aligned}
\end{equation}
and keeping the only commutator piece we get\\
\begin{equation}\label{eq:x}
    \begin{aligned}\frac{\lambda_{0}}{8} \frac{1}{\left(2 \pi\right)^{3}} \int d^{3}x \int d^{3}k \, \frac{\phi^{2}(x)}{\sqrt{k^{2}+m^{2}}}-\frac{\lambda_{0}}{8} \int d^{3}x \int_{k<M} \frac{d^{3}k}{(2\pi)^{3}} \, \frac{\phi(x)^{2}}{\sqrt{k^{2}+m^{2}}}.
    \end{aligned}
\end{equation}
Using dimensional regularization ($d=3-2\epsilon$), the result is\\
\begin{equation}\label{eq:x}
    \begin{aligned} &-\int d^{3}x \, \frac{\phi^{2}(x)}{2} \frac{\lambda_{0} m^{2}}{32 \pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right)+\frac{\lambda_{0}}{4}C\int d^{3}x \, \frac{\phi(x)^{2}}{2},\\
    & \frac{1}{\overline{\epsilon}}=\frac{1}{\epsilon}-\gamma+\ln{4\pi},\\
    &C=-\int_{k<M}\frac{d^{3}k}{(2\pi)^{3}}\,\frac{1}{\sqrt{k^{2}+m^{2}}}.
    \end{aligned}
\end{equation}
The term proportional to C is from the restriction imposed on the momentum of high frequency light field $\chi(x)$.\\
\indent Similarly, the Figure \ref{fig:ch31d} arises from the term\\
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{\lambda_{2}}{4} \int d^{3}x\, \sum_{k}\sum_{p} \frac{1}{\sqrt{2V\omega_{k}}}\frac{1}{\sqrt{2V\omega_{p}}} e^{i\left(\boldsymbol k - \boldsymbol p \right) \boldsymbol x} a_{k}a_{p}^{\dagger} \phi^{2}(x).
    \end{aligned}
\end{equation}
Normal ordering this term gives\\
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{\lambda_{2}}{4} \int d^{3}x\, \sum_{k}\sum_{p} \frac{1}{\sqrt{2V\omega_{k}}}\frac{1}{\sqrt{2V\omega_{p}}} e^{i\left(\boldsymbol k - \boldsymbol p \right) \boldsymbol x} \left(\left[a_{k},a_{p}^{\dagger} \right]+a_{p}^{\dagger}a_{k}\right) \phi^{2}(x).
    \end{aligned}
\end{equation}
Using dimensional regularization, we can get\\
\begin{equation}\label{eq:x}
    \begin{aligned} -\int d^{3}x \, \frac{\phi^{2}(x)}{2} \frac{\lambda_{2} M^{2}}{32 \pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{M^{2}}{\mu^{2}}}+1\right).
    \end{aligned}
\end{equation}
\indent Figure \ref{fig:ch31c} is proportional to $\lambda_{1}^{2}$ and $\phi^{2}$. Since it is second order in coupling constant, it must come from the term $\frac{i}{2}\left[H_{A}, \Omega_{0}\right]$ in eq.(3.6). To find the $H_{A}$ in this case, call it $H_{A}^{2,1}$ and consider the mode expansion of $\frac{\lambda_{1}}{2} \Phi_{H}\Phi_{L}^{2}$\\
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{\lambda_{1}}{2} \Phi_{H} \Phi_{L}^{2}&= \frac{\lambda_{1}}{2} \int d^{3}x \, \sum_{k} \sum_{M<p} \sum_{M<q} \frac{1}{\left(2V\right)^{\frac{3}{2}}\sqrt{\omega_{k}\epsilon_{p}\epsilon_{q}}} \left(a_{k} e^{i \boldsymbol k \boldsymbol x} + a_{k}^{\dagger} e^{-i \boldsymbol k \boldsymbol x}\right)\\ 
    &\left(b_{p} e^{i \boldsymbol p \boldsymbol x} + b_{p}^{\dagger} e^{-i \boldsymbol p \boldsymbol x} \right) \left(b_{q} e^{i \boldsymbol q \boldsymbol x} + b_{q}^{\dagger} e^{-i \boldsymbol q \boldsymbol x} \right)+\frac{\lambda_{1}}{2} \int d^{3}x \, \sum_{k} \frac{1}{\sqrt{2V\omega_{k}}}\\ &
    \phi^{2}(x)\left(a_{k} e^{i \boldsymbol k \boldsymbol x} + a_{k}^{\dagger} e^{-i \boldsymbol k \boldsymbol x}\right)+...
    \end{aligned}
\end{equation}
where dots represent terms proportional to $\phi(x)$.\\
\indent This expansion has a piece proportional to $\frac{\lambda_{1}}{2} \int d^{3}x \, \sum_{k} \frac{1}{\sqrt{2V\omega_{k}}} \left(a_{k} e^{i \boldsymbol k \boldsymbol x} + a_{k}^{\dagger} e^{-i \boldsymbol k \boldsymbol x}\right) \phi(x)^{2}$ in the $H_{A}^{2,1}$. In addition, there's another term, which is of the form of $H_{B}$:\\
\begin{equation}\label{eq:x}
    \begin{aligned} &\frac{\lambda_{1}}{2} \int d^{3}x \, \sum_{k} \sum_{M<p} \sum_{M<q} \frac{1}{\left(2V\right)^{\frac{3}{2}}\sqrt{\omega_{k}\epsilon_{p}\epsilon_{q}}} \left(a_{k} e^{i \boldsymbol k \boldsymbol x} + a_{k}^{\dagger} e^{-i \boldsymbol k \boldsymbol x}\right) b_{p} e^{i \boldsymbol p x} b_{q}^{\dagger} e^{-i \boldsymbol q \boldsymbol x}.\\
    \end{aligned}
\end{equation}
Normal ordering this gives,
\begin{equation}
    \begin{aligned} \frac{\lambda_{1}}{2} \int d^{3}x \, \sum_{k} \sum_{M<p} \sum_{M<q} \frac{1}{\left(2V\right)^{\frac{3}{2}}\sqrt{\omega_{k}\epsilon_{p}\epsilon_{q}}} \left(a_{k} e^{i \boldsymbol k \boldsymbol x} + a_{k}^{\dagger} e^{-i \boldsymbol k \boldsymbol x}\right) e^{i \left(\boldsymbol k -\boldsymbol p\right) \boldsymbol x} \left(\left[b_{p},b_{q}^{\dagger}\right]+b_{q}^{\dagger} b_{p}\right).
    \end{aligned}
\end{equation}
Finally, putting this together we get the net contribution of $H_{A}^{2,1}$ to be  
\begin{equation}\label{eq:x}
    \begin{aligned} H_{A}^{2,1} = \int d^{3}x \, \frac{\lambda_{1}}{2} \sum_{k} \frac{1}{\sqrt{2V\omega_{k}}} \left(a_{k} e^{i \boldsymbol k \boldsymbol x} + a_{k}^{\dagger} e^{-i \boldsymbol k \boldsymbol x}\right) \left(-\frac{m^{2}}{16 \pi^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right)+\frac{C}{2} +\phi(x)^{2}\right),
    \end{aligned}
\end{equation}
where again $C=-\int_{k<M}\frac{d^{3}k}{(2\pi)^{3}}\,\frac{1}{\sqrt{k^{2}+m^{2}}}$ and is from the restriction on $\chi(x)$'s momentum.
Denoting the contribution to $\Omega_{0}$ in this case by $\Omega_{0}^{2,1}$ we get from the condition that $i\left[H_{2},\Omega_{0}^{2,1}\right]+H_{A}^{2,1}=0$,\\
\begin{equation}\label{eq:x}
    \begin{aligned} \Omega_{0}^{2,1} = \int d^{3}y \, \frac{\lambda_{1}}{2} \sum_{p} \frac{-i}{\sqrt{2V\omega_{p}}\omega_{p}} \left(a_{p} e^{i \boldsymbol p \boldsymbol y} - a_{p}^{\dagger} e^{-i \boldsymbol p \boldsymbol y}\right) \left(-\frac{m^{2}}{16 \pi^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right)+\frac{C}{2} +\phi(y)^{2}\right).
    \end{aligned}
\end{equation}
Then we get,
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{i}{2}\left[H_{A}^{2,1},\Omega_{0}^{2,1}\right]=& -\frac{i}{2} \int \int d^{3}x d^{3}y \, \frac{\lambda_{1}^{2}}{4} \sum_{k} \sum_{p} \frac{-i}{2V\sqrt{\omega_{k} \omega_{p}}\omega_{p}} \left[a_{k},-a_{p}^{\dagger}\right] e^{i \boldsymbol k \boldsymbol x} e^{-i \boldsymbol p \boldsymbol y} \\& \left(\frac{m^{2}}{16 \pi^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right)-\frac{C}{2}\right) \phi(y)^{2} + \dots \\
    &= \int \int d^{3}x d^{3}y \, \frac{\lambda_{1}^{2}}{16} \sum_{k} \frac{1}{\omega_{k}^{2}} e^{i \boldsymbol k \left(\boldsymbol x - \boldsymbol y\right)}\left(\frac{m^{2}}{16 \pi^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right)-\frac{C}{2}\right) \phi(y)^{2}+\dots,\\
    \end{aligned}
\end{equation}
where the dots denote three other similar terms arising from the commutator.
Since momentum k is associated with external lines, we have $k \ll M$, and $\omega_{k}^{2} \simeq M^{2}$. Including all these contributions we get
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{i}{2}\left[H_{A}^{2,1},\Omega_{0}^{2,1}\right]&= \int \int d^{3}x d^{3}y \, \frac{4 \lambda_{1}^{2}}{16} \left(\frac{m^{2}}{16 \pi^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right)-\frac{C}{2}\right) \phi(y)^{2} \int \frac{d^{3}k}{\left(2 \pi  \right)^{3}} \, \frac{1}{M^{2}} e^{i \boldsymbol k \left(\boldsymbol x -\boldsymbol y\right)},\\
    &=  \int d^{3}x \, \frac{\lambda_{1}^{2}m^{2}}{32 \pi^{2} M^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right) \frac{\phi(x)^2}{2}-\frac{\lambda_{1}^{2}C}{4M^{2}}\int d^{3}x\, \frac{\phi(x)^{2}}{2}.
    \end{aligned}
\end{equation}
\indent Now let's consider Figure \ref{fig:ch31b} which is the last contribution to the two point function at one loop order. Figure \ref{fig:ch31b} has both light particle and heavy particle propagators. It arises also from the expansion of $\frac{\lambda_{1}}{2}\Phi_{H}\Phi_{L}^{2}$ and is not listed in eq.(3.14). This contribution is\\
\begin{equation}\label{eq:x}
    \begin{aligned} H_{A}^{2,2} = 2 \int d^{3}x \,  \sum_{k} \sum_{M<p} \frac{\lambda_{1}}{2} \frac{\phi(x)}{2V\sqrt{\omega_{k}\epsilon_{p}}} \left(a_{k} e^{i \boldsymbol k \boldsymbol x} b_{p} e^{i \boldsymbol p \boldsymbol x} + h.c. \right).
    \end{aligned}
\end{equation}
Similarly, from $i\left[H_{2},\Omega_{0}^{2,2}\right]+H_{A}^{2,2}=0$, we can get the $\Omega_{0}^{2,2}$ that corresponds to $H_{A}^{2,2}$,\\
\begin{equation}\label{eq:x}
    \begin{aligned} \Omega_{0}^{2,2} =2 \int d^{3}y \,  \sum_{q} \sum_{M<r} \frac{\lambda_{1}}{2} \left( \frac{-i \phi(x)}{2V\sqrt{\omega_{q}\epsilon_{r}} \left(\omega_{q}+\epsilon_{r}\right)} a_{q} e^{i \boldsymbol k \boldsymbol x} b_{r} e^{i \boldsymbol p \boldsymbol x} + h.c. \right).
    \end{aligned}
\end{equation}
Thus, we need to calculate $\frac{i}{2}\left[H_{A}^{2,2},\Omega_{0}^{2,2}\right]$. After a simple calculation, and normal ordering we can get:\\
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{i}{2}\left[H_{A}^{2,2},\Omega_{0}^{2,2}\right]&= - \int \int d^{3}x d^{3}y \, \sum_{k} \sum_{p<M} \lambda_{1}^{2} \frac{ \phi(x) \phi(y)}{4V^2\omega_{k}\epsilon_{p}\left(\omega_{k}+\epsilon_{p}\right)} e^{i \left(\boldsymbol k + \boldsymbol p\right) \left(\boldsymbol x - \boldsymbol y\right)},\\
    &= - \int \int d^{3}x d^{3}y \, \sum_{k} \sum_{p<M} \lambda_{1}^{2} \frac{ \phi(x) \phi(y)e^{i \left(\boldsymbol k + \boldsymbol p\right) \left(\boldsymbol x - \boldsymbol y\right)}}{4V^2\sqrt{k^{2}+M^{2}}\sqrt{p^{2}+m^{2}}\left(\sqrt{k^{2}+M^{2}}+\sqrt{p^{2}+m^{2}}\right)}.
    \end{aligned}
\end{equation}

In order to calculate this complicated integral, we need to split the forbidding fraction into two parts:
\begin{equation}\label{eq:x}
    \begin{aligned} & \frac{1}{\sqrt{k^{2}+M^{2}}\sqrt{p^{2}+m^{2}}\left(\sqrt{k^{2}+M^{2}}+\sqrt{p^{2}+m^{2}}\right)},\\
     =& \frac{\sqrt{k^{2}+M^{2}}-\sqrt{p^{2}+m^{2}}}{\sqrt{k^{2}+M^{2}}\sqrt{p^{2}+m^{2}}\left(k^{2}+M^{2}-p^{2}-m^{2}\right)},\\
     =& \frac{1}{\sqrt{p^{2}+m^{2}}\left(k^{2}+M^{2}-p^{2}-m^{2}\right)} - \frac{1}{\sqrt{k^{2}+M^{2}}\left(k^{2}+M^{2}-p^{2}-m^{2}\right)}.
    \end{aligned}
\end{equation}
Let $\boldsymbol k + \boldsymbol p = \boldsymbol r$. We know $\boldsymbol r$ is total external momentum, thus r is much smaller than M, which means $\left(k^{2}-p^{2}\right) \ll M^{2}$. Hence we can write:\\
\begin{equation}\label{eq:x}
    \begin{aligned} & \frac{1}{\sqrt{p^{2}+m^{2}}\left(k^{2}+M^{2}-p^{2}-m^{2}\right)},\\
     = &\frac{1}{\sqrt{p^{2}+m^{2}}M^{2}\left(1-\frac{m^{2}}{M^{2}}+\frac{k^{2}-p^{2}}{M^{2}}\right)},\\
     \simeq & \frac{1}{\sqrt{p^{2}+m^{2}}M^{2}}\left(1+\frac{m^{2}}{M^{2}}-\frac{k^{2}-p^{2}}{M^{2}}+\left(\frac{k^{2}-p^{2}}{M^{2}}\right)^{2}\right).
    \end{aligned}
\end{equation}
To the order $\frac{1}{M^{2}}$ this gives\\
\begin{equation}\label{eq:x}
    \begin{aligned} &\int d^{3}x \frac{m^{2}\lambda_{1}^{2}}{16\pi^{2}M^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right) \frac{\phi(x)^{2}}{2}-\frac{\lambda_{1}^{2}C}{2M^{2}}\int d^{3}x\,\frac{\phi(x)^{2}}{2}.
    \end{aligned}
\end{equation}
\indent Similarly, the second term from eq.(3.24) gives
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{1}{\sqrt{k^{2}+M^{2}}M^{2}}\left(1+\frac{m^{2}}{M^{2}}-\frac{k^{2}-p^{2}}{M^{2}}+\left(\frac{k^{2}-p^{2}}{M^{2}}\right)^{2}\right).
    \end{aligned}
\end{equation}
Straightforwardly, the first two terms in eq.(3.27) gives\\
\begin{equation}\label{eq:x}
    \begin{aligned} & \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \phi(y) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \int \frac{d^{3}r}{\left(2\pi\right)^{3}} \frac{1}{4 \sqrt{k^{2}+M^{2}}M^{2}} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)} \left(1+\frac{m^{2}}{M^{2}}\right),\\
    & = -\int d^{3}x \frac{\lambda_{1}^{2}}{16\pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{M^{2}}{\mu^{2}}}+1\right) \frac{\phi(x)^{2}}{2} \left(1+\frac{m^{2}}{M^{2}}\right).
    \end{aligned}
\end{equation}
The last two terms are a bit tricky to handle. First, we need to do some modification\\
\begin{equation}\label{eq:x}
    \begin{aligned} k^{2}-p^{2} &= \left(\boldsymbol k + \boldsymbol p\right) \left(\boldsymbol k -\boldsymbol p\right),\\
    & = 2\boldsymbol k \boldsymbol r - r^{2}.
    \end{aligned}
\end{equation}
Then we have from the $\frac{k^{2}-p^{2}}{M^{2}}$ term:\\
\begin{equation}\label{eq:x}
    \begin{aligned}& \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \phi(y) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \int \frac{d^{3}r}{\left(2\pi\right)^{3}} \frac{1}{4 \sqrt{k^{2}+M^{2}}M^{2}} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)} \left(-\frac{k^{2}-p^{2}}{M^{2}}\right),\\
    & = \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \phi(y) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \int \frac{d^{3}r}{\left(2\pi\right)^{3}} \frac{1}{4 \sqrt{k^{2}+M^{2}}M^{2}} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)} \left(\frac{-2 \boldsymbol k \boldsymbol r +r^{2}}{M^{2}}\right),\\
    & =  \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \phi(y) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \int \frac{d^{3}r}{\left(2\pi\right)^{3}} \frac{1}{4 \sqrt{k^{2}+M^{2}}M^{2}} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)}\frac{r^{2}}{M^{2}},\\
    & = \int \int d^{3}(x) d^{3}(y) \, \frac{\lambda_{1}^{2}}{4} \phi(x) \phi(y) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \frac{1}{M^{2}\sqrt{k^{2}+M^{2}}} \int \frac{d^{3}r}{\left(2\pi\right)^{3}} r^{2} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)},\\
    & = \int \int d^{3}(x) d^{3}(y) \, \frac{\lambda_{1}^{2}}{4} \phi(x) \phi(y) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \frac{1}{M^{2}\sqrt{k^{2}+M^{2}}} \left(\delta^{3}(\boldsymbol x -\boldsymbol y) \partial_{y}^{2}\right),\\
    & = \int d^{3}(x) \, \frac{\lambda_{1}^{2}}{4} \phi(x) \partial^{2} \phi(x) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \frac{1}{M^{2}\sqrt{k^{2}+M^{2}}},\\
    & = \int d^{3}(x) \, \frac{\lambda_{1}^{2}}{16\pi^{2}M^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{M^{2}}{\mu^{2}}}+1\right) \frac{1}{2}(\partial \phi(x))^{2}.
    \end{aligned}
\end{equation}
To the order $\frac{2}{M^{2}}$, we also need to consider the $\frac{4\left(\boldsymbol k \boldsymbol r\right)^{2}}{M^{4}}$ term from $\left(\frac{k^{2}-p^{2}}{M^{2}}\right)^{2}$:
\begin{equation}\label{eq:x}
    \begin{aligned} & \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \phi(y) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \int \frac{d^{3}r}{\left(2\pi\right)^{3}} \frac{1}{4 \sqrt{k^{2}+M^{2}}M^{2}} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)}\frac{4\left(\boldsymbol k \boldsymbol r\right)^{2}}{M^{4}},\\ 
    & = \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \phi(y) \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \frac{1}{ \sqrt{k^{2}+M^{2}}M^{6}} \int \frac{d^{3}r}{\left(2\pi\right)^{3}} \left(\boldsymbol k \boldsymbol r\right)^{2} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)},\\
    & =  \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \phi(y) \int \frac{d^{3}r}{\left(2\pi\right)^{3}} r^{2} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)} \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \frac{k^{2}\cos^{2}{\theta}}{\sqrt{k^{2}+M^{2}}M^{6}},\\
    & = \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \phi(y) \int \frac{d^{3}r}{\left(2\pi\right)^{3}} r^{2} e^{i \boldsymbol r \left(\boldsymbol x - \boldsymbol y\right)} \frac{1}{32\pi^{2}M^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{M^{2}}{\mu^{2}}}+\frac{3}{2}\right),\\
    & = \int \int d^{3}x d^{3} y \, \lambda_{1}^{2} \phi(x) \delta^{3}(\boldsymbol x- \boldsymbol y) \partial_{y}^{2} \phi(y) \frac{1}{32\pi^{2}M^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{M^{2}}{\mu^{2}}}+\frac{3}{2}\right),\\
    & = -\int d^{3}x\, \frac{\lambda_{1}^{2}}{16\pi^{2}M^{2}} \left(\frac{1}{\overline{\epsilon}}-\ln{\frac{M^{2}}{\mu^{2}}}+\frac{3}{2}\right) \frac{1}{2} (\partial \phi(x))^{2}.
    \end{aligned}
\end{equation}
Putting together all the previous results, we can get the total contribution from Figure \ref{fig:ch31b} as\\
\begin{equation}\label{eq:x}
    \begin{aligned} 
    &\frac{m^{2}\lambda_{1}^{2}}{16\pi^{2}M^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1\right)\int d^{3}x\, \frac{\phi(x)^{2}}{2}-\frac{\lambda_{1}^{2}C}{2M^{2}}\int d^{3}x\,\frac{\phi(x)^{2}}{2}\\
    &-\frac{\lambda_{1}^{2}}{16\pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{M^{2}}{\mu^{2}}}+1\right)\left(1+\frac{m^{2}}{M^{2}}\right)\int d^{3}x \, \frac{\phi(x)^{2}}{2} -\frac{\lambda_{1}^{2}}{32\pi^{2}M^{2}}\int d^{3}x\,\frac{1}{2} (\partial \phi(x))^{2}.
    \end{aligned}
\end{equation}
Putting contributions from all the diagrams together and taking $\mu \approx M$ to get rid of log terms $\ln{\frac{M^{2}}{\mu^{2}}}$, we have the net result of two point functions as
\begin{equation}
    \begin{aligned}
    &-\frac{\lambda_{0}m^{2}}{32\pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{M^{2}}}+1\right)\int d^{3}x\, \frac{\phi(x)^{2}}{2}-\frac{\lambda_{2}M^{2}}{32\pi^{2}}\left(\frac{1}{\overline{\epsilon}}+1\right)\int d^{3}x\, \frac{\phi(x)^{2}}{2}\\
    &+\frac{3\lambda_{1}^{2}m^{2}}{32\pi^{2}M^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{M^{2}}}+1\right)\int d^{3}x\, \frac{\phi(x)^{2}}{2}-\frac{\lambda_{1}^{2}}{16\pi^{2}}\left(\frac{1}{\overline{\epsilon}}+1\right)\left(1+\frac{m^{2}}{M^{2}}\right)\int d^{3}x\, \frac{\phi(x)^{2}}{2}\\
    &-\frac{\lambda_{1}^{2}}{32\pi^{2}M^{2}}\int d^{3}x\,\frac{1}{2} (\partial \phi(x))^{2}+\left(\frac{\lambda_{0}C}{4}-\frac{3\lambda_{1}^{2}C}{2M^{2}}\right)\int d^{3}x\,\frac{\phi(x)^{2}}{2}.
    \end{aligned}
\end{equation}
\indent There are several finite contributions proportional to $C=-\int_{k<M}\frac{d^{3}k}{(2\pi)^{3}}\,\frac{1}{\sqrt{k^{2}+m^{2}}}$, however they will not affect the renormalization of $H_{1}$ as we will show in section \ref{subsec:ch33}. In fact, they will only appear in $H_{decoupled}$ and get canceled out in the physical effective Hamiltonian $H_{eff}$ during the matching which will be shown in chapter \ref{sec:EFT}. Another way to think about the effects of these finite terms is that whenever we have a light field in the loop, our calculation will produce these finite terms along with (in a linear way) the "troublesome" large log terms $\ln{\frac{m^{2}}{M^{2}}}$. Therefore, as long as the large log terms can be canceled during matching, we can persuade ourselves that these extra finite terms will get canceled and will not appear in $H_{eff}$ as well.
\subsubsubsection{Four Point Function Calculation }
\label{subsubsec:ch322}
\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{Figures/4pt2.png}
    \caption{\label{fig:4pt} Four point function at tree level.}
\end{figure}
In the calculation of Figure \ref{fig:ch31c} in section \ref{subsubsec:ch321}, there is one more term from the commutator $\frac{i}{2}\left[H_{A}^{2,1},\Omega_{0}^{2,1}\right]$ left undiscussed that contributes to the four point function at tree level shown in Figure \ref{fig:4pt}
\begin{equation}
    \begin{aligned} \frac{i}{2}\left[H_{A}^{2,1},\Omega_{0}^{2,1}\right]_{tree}&=i\int d^{3}x \int d^{3} y \,\frac{\lambda_{1}^{2}}{4} \sum_{k} \sum_{p} \frac{-i}{2V\sqrt{\omega_{k}\omega_{p}}\omega_{p}}\phi(x)^{2}\phi(y)^{2}[a_{k},-a_{p}^{\dagger}]e^{i\boldsymbol{kx}-i\boldsymbol{py}},\\
    &=-\int d^{3}x\int d^{3}y \int \frac{d^{3}k}{(2\pi)^{3}}\frac{\lambda_{1}^{2}}{8(k^{2}+M^{2})}\phi(x)^{2}\phi(y)^{2}e^{i\boldsymbol{k}(\boldsymbol{x}-\boldsymbol{y})},\\
    &\approx -\frac{3\lambda_{1}}{M^{2}}\int d^{3}x\,\frac{\phi(x)^{4}}{4 !},
    \end{aligned}
\end{equation}
where we have used the condition that k is associated with external momenta and therefore $k\ll M$.\\
\begin{figure}[tbp]
\centering 
\subfigure[]{\includegraphics[width=.2\textwidth]{4a.png}\label{fig:ch33a}}
\hfill
\subfigure[]{\includegraphics[width=.2\textwidth]{4B.png}\label{fig:ch33b}}
\hfill
\subfigure[]{\includegraphics[width=.3\textwidth]{4C.png}\label{fig:ch33c}}
\hfill
\subfigure[]{\includegraphics[width=.2\textwidth]{4D.png}\label{fig:ch33d}}
\caption{\label{fig:i} Four point functions at one loop level.}
\end{figure}
\indent In the loop calculation we will encounter extra finite terms similar to those we have discussed in section \ref{subsubsec:ch321}. However we will omit them in our calculation and check in chapter \ref{sec:EFT} that all the large log terms $\ln{\frac{m^{2}}{M^{2}}}$ produced in four point function calculation are canceled out, which implies these extra finite terms will be canceled too. Furthermore, we will set external momenta to 0, an assumption that will simplify calculation greatly but won't damage the physical essence of our theory.\\
\indent Let's consider Figure \ref{fig:ch33a}. This diagram is of order $\lambda_{0}^{2}$, and it arises from the term $\frac{i}{2} \left[H_{A}^{4,1},\Omega_{0}^{4,1}\right]$ where $H_{A}^{4,1}$ comes from the mode expansion of $\frac{\lambda_0}{4!}\Phi_{L}(x)^{4}$. In this expansion we must pick a term of form $\phi^{2}\chi^{2}$ which gives
\begin{equation}\label{eq:x}
    \begin{aligned} H_{A}= \int d^{3}x \, 6 \frac{\lambda_{0}}{4!} \phi(x)^{2} \sum_{k}\sum_{p} \frac{1}{2V\sqrt{\epsilon_{p}\epsilon_{k}}}\left(b_{p} b_{k} e^{i\left(\boldsymbol p + \boldsymbol k\right)\boldsymbol x}+b_{p}^{\dagger}b_{k}^{\dagger}e^{-i\left(\boldsymbol p + \boldsymbol k\right)\boldsymbol x}\right).
    \end{aligned}
\end{equation}
From the equation $i\left[H_{2},\Omega_{0}^{4,1}\right]+H_{A}^{4,1}=0$, we can get the corresponding $\Omega_{0}^{4,1}$ to be
\begin{equation}\label{eq:x}
    \begin{aligned} \Omega_{0}^{4,1} = \int d^{3}y \, \frac{\lambda_{0}}{4} \phi(y)^{2} \sum_{k^{'}} \sum_{p^{'}} \left(\frac{-i e^{i\left(\boldsymbol k^{'}+\boldsymbol p^{'}\right)\boldsymbol y}}{2V\sqrt{\epsilon_{k^{'}}\epsilon_{p^{'}}}\left(\epsilon_{k^{'}}+\epsilon_{p^{'}}\right)}b_{k^{'}}b_{p^{'}}+\frac{i e^{-i\left(\boldsymbol k^{'}+\boldsymbol p^{'}\right)\boldsymbol y}}{2V\sqrt{\epsilon_{k^{'}}\epsilon_{p^{'}}}\left(\epsilon_{k^{'}}+\epsilon_{p^{'}}\right)}b_{k^{'}}^{\dagger}b_{p^{'}}^{\dagger}\right).
    \end{aligned}
\end{equation}
Then $\frac{i}{2} \left[H_{A}^{4,1},\Omega_{0}^{4,1}\right]$ yields
\begin{equation}\label{eq:x}
    \begin{aligned}  -\frac{3\lambda_{0}^{2}}{32\pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln\frac{m^{2}}{\mu^{2}}\right)\int d^{3}x \, \frac{\phi(x)^{4}}{4!}.
    \end{aligned}
\end{equation}
In this calculation, we have used the approximation that total external momentum is zero, which means $\boldsymbol k +\boldsymbol p = 0$ and $\epsilon_{k} = \epsilon_{p} = \sqrt{k^{2}+m^{2}}$.\\ 
\indent The next contribution is from Figure \ref{fig:ch33b}. The calculation is similar to the first one except the corresponding $H_{A}$ is different. In this case we have 

\begin{subequations}\label{eq:y}
\begin{align}
\label{eq:y:1}
&H_{A}^{4,2}= \int d^{3}x \,  \frac{\lambda_{2}}{4} \phi(x)^{2} \sum_{k}\sum_{p} \frac{1}{2V\sqrt{\omega_{p}\omega_{k}}}\left(a_{p} a_{k} e^{i\left(\boldsymbol p + \boldsymbol k\right)\boldsymbol x}+a_{p}^{\dagger}a_{k}^{\dagger}e^{-i\left(\boldsymbol p + \boldsymbol k\right)\boldsymbol x}\right),\\
\label{eq:y:2}
&\Omega_{0}^{4,2} = \int d^{3}y \, \frac{\lambda_{2}}{4} \phi(y)^{2} \sum_{k^{'}} \sum_{p^{'}} \left(\frac{-i e^{i\left(\boldsymbol k^{'}+\boldsymbol p^{'}\right)\boldsymbol y}}{2V\sqrt{\omega_{k^{'}}\omega_{p^{'}}}\left(\omega_{k^{'}}+\omega_{p^{'}}\right)}a_{k^{'}}a_{p^{'}}+\frac{i e^{-i\left(\boldsymbol k^{'}+\boldsymbol p^{'}\right)\boldsymbol y}}{2V\sqrt{\omega_{k^{'}}\omega_{p^{'}}}\left(\omega_{k^{'}}+\omega_{p^{'}}\right)}a_{k^{'}}^{\dagger}a_{p^{'}}^{\dagger}\right).
\end{align}
\end{subequations}
Following the similar calculation we are able to get the result:
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{i}{2} \left[H_{A}^{4,2},\Omega_{0}^{4,2}\right] = -\frac{3\lambda_{2}^{2}}{32\pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln\frac{M^{2}}{\mu^{2}}\right)\int d^{3}x \, \frac{\phi(x)^{4}}{4!}.
    \end{aligned}
\end{equation}
\begin{table}[t]
    \centering
    \begin{tabular}{|lll|} 
    \hline
    $H_{A}^{4,3}$ &$\Omega_{0}^{4,3,1}$& $\Omega_{0}^{4,3,2}$ \\ \hline  
    First combination (a) & & \\ 
    $\lambda_{1}a\phi^{2}$ &  $\lambda_{1}a^{\dagger}b^{\dagger}b^{\dagger}$ & $\lambda_{0}bb\phi^{2}$\\
    $\lambda_{1}a^{\dagger}\phi^{2}$ & $\lambda_{1}abb$ & $\lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$\\ \hline
    Second combination (b) & & \\
    $\lambda_{1}abb$ & $ \lambda_{1}a^{\dagger}\phi^{2}$ & $\lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$\\
    $\lambda_{1}a^{\dagger}b^{\dagger}b^{\dagger}$ & $\lambda_{1}a\phi^{2}$ & $ \lambda_{0}bb\phi^{2}$\\ \hline
    Third combination (c) & &\\
    $\lambda_{1}abb$ & $\lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$ & $\lambda_{1}a^{\dagger}\phi^{2}$\\
    $\lambda_{1}a^{\dagger}b^{\dagger}b^{\dagger}$ & $\lambda_{0}bb\phi^{2}$ & $\lambda_{1}a\phi^{2}$\\ \hline
    Fourth combination (d) & &\\
    $\lambda_{0}bb\phi^{2}$ & $\lambda_{1}a^{\dagger}b^{\dagger}b^{\dagger}$ & $\lambda_{1}a\phi^{2}$\\
    $\lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$ & $\lambda_{1}abb$ & $\lambda_{1}a^{\dagger}\phi^{2}$ \\ \hline
    \end{tabular}
    \caption{Combinations of $-\frac{1}{3}\left[\left[H_{A}^{4,3},\Omega_{0}^{4,3,1}\right],\Omega_{0}^{4,3,2}\right]$ that contribute to Figure \ref{fig:ch33c}.}
    \label{tab:ch31}
\end{table}
\indent Let's now consider the contributions that correspond to Figure \ref{fig:ch33c}.
Notice that, in this diagram, we have the product of coupling constants as $\lambda_{0}\lambda_{1}^{2}$, which means we need $-\frac{1}{3}\left[\left[H_{A},\Omega_{0}\right],\Omega_{0}\right]-\frac{1}{2}\left[\left[H_{B},\Omega_{0}\right],\Omega_{0}\right]$ from eq.(3.6). For clarity, we label $H_{A}$ in the commutator as $H_{A}^{4,3}$, the first $\Omega_{0}$ next to $H_{A}^{4,3}$ as $\Omega_{0}^{4,3,1}$, the second $\Omega_{0}$ as $\Omega_{0}^{4,3,2}$ and $H_{B}$ as $H_{B}^{4,3}$. There are many ways to pick $H_{A}^{4,3}$, $\Omega_{0}^{4,3,1}$, and $\Omega_{0}^{4,3,2}$ in $-\frac{1}{3} \left[\left[H_{A}^{4,3},\Omega_{0}^{4,3,1}\right],\Omega_{0}^{4,3,2}\right]$, and we split them into four kinds of combinations shown in Table \ref{tab:ch31}. We will show the explicit calculation of the first combination Table \ref{tab:ch31}(a) and put the calculation of other combinations in the appendix \ref{sec:app3}.\\
\indent Considering the following terms from the first combination Table \ref{tab:ch31}(a):
\begin{subequations}\label{eq:y}
\begin{align}
\label{eq:y:1}
H_{A}^{4,3} &= \frac{\lambda_{1}}{2} \int d^{3}x \, \sum_{k} \frac{\phi(x)^{2}}{\sqrt{2V\omega_{k}}} a_{k}e^{i \boldsymbol k \boldsymbol x},
\\
\label{eq:y:2}
\Omega_{0}^{4,3,1} &= \frac{\lambda_{1}}{2} \int d^{3}y \, \sum_{k^{'}} \sum_{p} \sum_{q} 
\frac{i e^{-i\left(\boldsymbol k^{'} + \boldsymbol p + \boldsymbol q\right) \boldsymbol y}}{\left(2V\right)^{3/2}\sqrt{\omega_{k^{'}}\epsilon_{p}\epsilon_{q}}\left(\omega_{k^{'}}+\epsilon_{p}+\epsilon_{q}\right)}a_{k^{'}}^{\dagger}b_{p}^{\dagger}b_{q}^{\dagger},
\\
\label{eq:y:3}
\Omega_{0}^{4,3,2} &= \frac{\lambda_{0}}{4} \int d^{3}z \, \sum_{p^{'}} \sum_{q^{'}} \phi(z)^{2} \frac{-i e^{i\left(\boldsymbol p^{'} +\boldsymbol q^{'}\right)\boldsymbol z}}{2V\sqrt{\epsilon_{p^{'}}\epsilon_{q^{'}}}\left(\epsilon_{p^{'}}+\epsilon_{q^{'}}\right)}b_{p^{'}}b_{q^{'}}.
\end{align}
\end{subequations}
We first calculate $\left[H_{A}^{4,3},\Omega_{0}^{4,3,1}\right]$
\begin{equation}\label{eq:x}
    \begin{aligned} \left[H_{A}^{4.3},\Omega_{0}^{4,3,1}\right] &= \frac{\lambda_{1}^{2}}{4} \int d^{3}x \int d^{3}y \, \phi(x)^{2} \sum_{k}\sum_{k^{'}}\sum_{p}\sum_{q} \frac{i e^{i \boldsymbol k \boldsymbol x} e^{-i\left(\boldsymbol k^{'} + \boldsymbol p + \boldsymbol q\right) \boldsymbol y} }{\left(2V\right)^{2}\sqrt{\omega_{k}\omega_{k^{'}}\epsilon_{p}\epsilon_{q}}\left(\omega_{k^{'}}+\epsilon_{p}+\epsilon_{q}\right)}\\& \left[a_{k},a_{k^{'}}^{\dagger}b_{p}^{\dagger}b_{q}^{\dagger}\right],\\
    & = \frac{\lambda_{1}^{2}}{4} \int d^{3}x \int d^{3}y \, \phi(x)^{2}\sum_{k}\sum_{p}\sum_{q} \frac{i e^{i \boldsymbol k \left(\boldsymbol x - \boldsymbol y\right)} e^{-i\left( \boldsymbol p + \boldsymbol q\right) \boldsymbol y} }{\left(2V\right)^{2}\omega_{k}\sqrt{\epsilon_{p}\epsilon_{q}}\left(\omega_{k^{}}+\epsilon_{p}+\epsilon_{q}\right)} b_{p}^{\dagger} b_{q}^{\dagger},\\
    & = \frac{i\lambda_{1}^{2}}{16} \int d^{3}x \, \phi(x)^{2} \sum_{p} \sum_{q} \frac{e^{-i\left(\boldsymbol p + \boldsymbol q\right)\boldsymbol x }}{VM\sqrt{\epsilon_{p}\epsilon_{q}}\left(M+\epsilon_{p}+\epsilon_{q}\right)}b^{\dagger}_{p}b^{\dagger}_{q}.
    \end{aligned}
\end{equation}
In the above calculation, we also use the assumption that total external momentum is 0, which implies the momentum $k$ associated with heavy particle is therefore 0 and $w_{k} = M$.
Then we have
\begin{equation}\label{eq:x}
    \begin{aligned} -\frac{1}{3}\left[\left[H_{A}^{4,3},\Omega_{0}^{4,3,1}\right],\Omega_{0}^{4,3,2}\right] &= -\frac{\lambda_{1}^{2}\lambda_{0}}{192} \int d^{3}x \int d^{3}z \,\sum_{p}\sum_{q}\sum_{p^{'}}\sum_{q^{'}} \phi(x)^{2}\phi(z)^{2}\\
    & \frac{e^{i\left(\boldsymbol p^{'} + \boldsymbol q^{'}\right)\boldsymbol z -i\left(\boldsymbol p + \boldsymbol q\right)\boldsymbol x}}{2V^{2}M\sqrt{\epsilon_{p}\epsilon_{q}\epsilon_{p^{'}}\epsilon_{q^{'}}}\left(\epsilon_{p^{'}}+\epsilon_{q^{'}}\right)\left(M+\epsilon_{p}+\epsilon_{q}\right)} \left[b_{p}^{\dagger}b_{q}^{\dagger},b_{p^{'}}b_{q^{'}}\right],\\
    &= \frac{\lambda_{1}^{2}\lambda_{0}}{192} \int d^{3}x \int d^{3}z \,\sum_{p} \sum_{q} \phi(x)^{2} \phi(z)^{2} \frac{e^{i\left(\boldsymbol p + \boldsymbol q\right)\left(\boldsymbol x - \boldsymbol z\right)}}{2V^{2}M\epsilon_{p}^{3}\left(M+2\epsilon{p}\right)},\\
    &= \frac{\lambda_{1}^{2}\lambda_{0}}{192} \int d^{3}x \, \phi(x)^{4} \int\frac{d^{3}p}{\left(2\pi\right)^{3}}\,\frac{1}{2V^{2}M\epsilon_{p}^{3}\left(M+2\epsilon_{p}\right)},
    \end{aligned}
\end{equation}
where we have used the fact that $\boldsymbol p +\boldsymbol q = \boldsymbol k = 0$, and thus $\epsilon_{p}=\epsilon_{q}$. Finally, taking the Hermitian conjugation into consideration, we have the result of combination Table \ref{tab:ch31}(a) to be
\begin{equation}\label{eq:x}
    \frac{\lambda_{1}^{2}\lambda_{0}}{96}\int d^{3}x \, \phi(x)^{4} \int\frac{d^{3}p}{\left(2\pi\right)^{3}}\,\frac{1}{2V^{2}M\epsilon_{p}^{3}\left(M+2\epsilon_{p}\right)}.
\end{equation}
\indent Combinations Table \ref{tab:ch31}(b) and Table \ref{tab:ch31}(c) will yield the same result:
\begin{equation}
    \begin{aligned} \frac{\lambda_{1}^{2}\lambda_{0}}{96}\int d^{3}x \, \phi(x)^{4} \int \frac{d^{3}p}{(2\pi)^{3}}\, \frac{1}{2M^{2}\epsilon_{p}^{3}}.
    \end{aligned}
\end{equation}
\indent Table \ref{tab:ch31}(d) will give
\begin{equation}
    \begin{aligned} \frac{\lambda_{1}^{2}\lambda_{0}}{96}\int d^{3}x \, \phi(x)^{4} \int \frac{d^{3}p}{(2\pi)^{3}}\, \frac{1}{M^{2}\epsilon_{p}^{2}(M+2\epsilon_{p})}.
    \end{aligned}
\end{equation}
\indent Adding all four kinds of combinations together, we will get 
\begin{equation}\label{eq:x}
    \begin{aligned} &\frac{\lambda_{1}^{2}\lambda_{0}}{96}\int d^{3}x \, \phi(x)^{4} \int \frac{d^{3}p}{\left(2\pi\right)^{3}} \, \left(\frac{1}{M^{2}\epsilon_{p}^{2}\left(M+2\epsilon_{p}\right)}+\frac{1}{2\epsilon_{p}^{3}M\left(M+2\epsilon_{p}\right)}+\frac{1}{M^{2}\epsilon_{p}^{3}}\right),\\
    &=\frac{\lambda_{1}^{2}\lambda_{0}}{64} \int d^{3}x \phi(x)^{4} \int \frac{d^{3}p}{\left(2\pi\right)^{3}}\,\frac{1}{M^{2}\epsilon_{p}^{3}},\\
    &= \frac{3\lambda_{1}^{2}\lambda_{0}}{32\pi^{2}M^{2}} \int d^{3}x \, \frac{\phi(x)^{4}}{4!} \left(\frac{1}{\overline{\epsilon}}-\ln\frac{m^{2}}{\mu^{2}}\right).
    \end{aligned}
\end{equation}
\begin{table}[t]
    \centering
    \begin{tabular}{|lll|} 
    \hline
    $H_{B}^{4,3}$ &$\Omega_{0}^{4,3,1}$& $\Omega_{0}^{4,3,2}$ \\ \hline  
    $\lambda_{1}b^{\dagger}b^{\dagger}a$ & $\lambda_{0}bb\phi^{2}$ & $\lambda_{1}a^{\dagger}\phi$ \\
    $\lambda_{1}b^{\dagger}b^{\dagger}a$ & $\lambda_{1}a^{\dagger}\phi^{2}$ & $\lambda_{0}bb\phi^{2}$ \\
    $\lambda_{1}a^{\dagger}bb$ & $\lambda_{1}a\phi^{2}$ & $\lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$ \\
    $\lambda_{1}a^{\dagger}bb$ & $\lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$ & $\lambda_{1}a\phi^{2}$ \\
    \hline
    \end{tabular}
    \caption{Combinations of $-\frac{1}{2}\left[\left[H_{B}^{4,3},\Omega_{0}^{4,3,1}\right],\Omega_{0}^{4,3,2}\right]$ that contribute to Figure \ref{fig:ch33c}.}
    \label{tab:ch32}
\end{table}
The combinations of $-\frac{1}{2}\left[\left[H_{B}^{4,3},\Omega_{0}^{4,3,1}\right],\Omega_{0}^{4,3,2}\right]$ are shown in Table \ref{tab:ch32}, and the result is 
\begin{equation}
    \begin{aligned} \frac{3\lambda_{1}^{2}\lambda_{0}}{32\pi^{2}M^{2}} \int d^{3}x \, \frac{\phi(x)^{4}}{4!} \left(\frac{1}{\overline{\epsilon}}-\ln\frac{m^{2}}{\mu^{2}}\right).
    \end{aligned}
\end{equation}
Therefore, the total contribution from Figure \ref{fig:ch33c} is 
\begin{equation}
    \begin{aligned} \frac{3\lambda_{1}^{2}\lambda_{0}}{16\pi^{2}M^{2}} \int d^{3}x \, \frac{\phi(x)^{4}}{4!} \left(\frac{1}{\overline{\epsilon}}-\ln\frac{m^{2}}{\mu^{2}}\right).
    \end{aligned}
\end{equation}
\begin{table}[t]
    \centering
    \begin{tabular}{|lll|} 
    \hline
    $H_{B}^{4,4}$ &$\Omega_{0}^{4,4,1}$& $\Omega_{0}^{4,4,2}$ \\ \hline  
    First combination (a) & & \\ 
    $\lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$ &  $\lambda_{1}a^{\dagger}b^{\dagger}\phi$ & $\lambda_{1}ab\phi$\\
    $\lambda_{0}b^{\dagger}b\phi^{2}$ & $\lambda_{1}ab\phi$ & $\lambda_{1}a^{\dagger}b^{\dagger}\phi$\\ \hline
    Second combination (b) & & \\
    $\lambda_{1}b^{\dagger}a\phi$ & $ \lambda_{1}a^{\dagger}b^{\dagger}\phi$ & $\lambda_{0}bb\phi^{2}$\\
    $\lambda_{1}a^{\dagger}b\phi$ & $\lambda_{1}ab\phi$ & $ \lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$\\ \hline
    Third combination (c) & &\\
    $\lambda_{1}b^{\dagger}a\phi$ & $\lambda_{0}bb\phi^{2}$ & $\lambda_{1}a^{\dagger}b^{\dagger}\phi$\\
    $\lambda_{1}a^{\dagger}b^{\dagger}\phi$ & $\lambda_{0}b^{\dagger}b^{\dagger}\phi^{2}$ & $\lambda_{1}ab\phi$\\ \hline
    \end{tabular}
    \caption{Combinations of $-\frac{1}{2}\left[\left[H_{B}^{4,4},\Omega_{0}^{4,4,1}\right],\Omega_{0}^{4,4,2}\right]$ that contribute to Figure \ref{fig:ch33c}.}
    \label{tab:ch33}
\end{table}
\indent As for the Figure \ref{fig:ch33d}, only the term  $-\frac{1}{2}\left[\left[H_{B}^{4,4},\Omega_{0}^{4,4,1}\right],\Omega_{0}^{4,4,2}\right]$ will contribute. Similarly, we divide the whole commutator into several kinds of combinations shown in Table \ref{tab:ch33} and calculate them respectively. We will give the resul of each kind of combination directly and put the explicit calculation in appendix \ref{sec:app3}.\\
\indent Table \ref{tab:ch33}(a) will give
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{\lambda_{0}\lambda_{1}^{2}}{16} \int d^{3}x  \, \phi(x)^{4} \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \frac{1}{\omega_{k}\epsilon_{k}^{2}\left(\omega_{k}+\epsilon_{k}\right)^{2}}.
    \end{aligned}
\end{equation}
\indent Since Table \ref{tab:ch33}(b) and Table \ref{tab:ch33}(c) only differ from an exchange of $\Omega_{0}^{4,4,1}$ and $\Omega_{0}^{4,4,2}$, they will give the same result:
\begin{equation}\label{eq:x}
    \begin{aligned} \frac{\lambda_{1}^{2}\lambda_{0}}{32} \int d^{3}x \, \phi(x)^{4} \int \frac{d^{3}p}{\left(2\pi\right)^{3}} \, \frac{1}{\omega_{p}\epsilon_{p}^{3}\left(\omega_{p}+\epsilon_{p}\right)}.
    \end{aligned}
\end{equation}
\indent Adding all three results together we will have
\begin{equation}\label{eq:x}
    \begin{aligned} -\frac{1}{2}\left[\left[H_{B}^{4,4},\Omega_{0}^{4,4,1}\right],\Omega_{0}^{4,4,2}\right] = \frac{\lambda_{1}^{2}\lambda_{0}}{16} \int d^{3}x \, \phi(x)^{4} \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \, \left[\frac{1}{\omega_{k}\epsilon_{k}^{2}\left(\omega_{k}+\epsilon_{k}\right)^{2}}+\frac{1}{\omega_{k}\epsilon_{k}^{3}\left(\omega_{k}+\epsilon_{k}\right)}\right].
    \end{aligned}
\end{equation}
Let's consider $\int \frac{d^{3}k}{\left(2\pi\right)^{3}} \frac{1}{\omega_{k}\epsilon_{k}^{3}\left(\omega_{k}+\epsilon_{k}\right)} $ first,
\begin{equation}\label{eq:x}
    \begin{aligned} \int \frac{d^{3}k}{\left(2\pi\right)^{3}}\, \frac{1}{\omega_{k}\epsilon_{k}^{3}\left(\omega_{k}+\epsilon_{k}\right)} &=  \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \, \left(\frac{1}{\epsilon^{3}_{k}\left(M^{2}-m^{2}\right)}-\frac{1}{\omega_{k}\epsilon_{k}^{2}\left(\omega_{k}+\epsilon_{k}\right)\left(\omega_{k}-\epsilon_{k}\right)}\right),\\
    &\approx \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \, \left(\frac{1}{\epsilon^{3}_{k}M^{2}}-\frac{1}{\omega_{k}\epsilon_{k}^{2}\left(\omega_{k}+\epsilon_{k}\right)\left(\omega_{k}-\epsilon_{k}\right)}\right).
    \end{aligned}
\end{equation}
Calculation of $\int \frac{d^{3}k}{\left(2\pi\right)^{3}} \, \frac{1}{\epsilon^{3}_{k}M^{2}}$ is straightforward, and we save it for later. Now consider
\begin{equation}\label{eq:x}
    \begin{aligned} &\int \frac{d^{3}k}{\left(2\pi\right)^{3}} \, \left(\frac{1}{\omega_{k}\epsilon_{k}^{2}\left(\omega_{k}+\epsilon_{k}\right)^{2}}-\frac{1}{\omega_{k}\epsilon_{k}^{2}\left(\omega_{k}+\epsilon_{k}\right)\left(\omega_{k}-\epsilon_{k}\right)}\right),\\
    &= \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \, \frac{-2\epsilon_{k}}{\omega_{k}\epsilon_{k}^{2}\left(\omega_{k}+\epsilon_{k}\right)^{2}\left(\omega_{k}-\epsilon_{k}\right)},\\
    &=\int \frac{d^{3}k}{\left(2\pi\right)^{3}} \, \frac{-2\epsilon_{k}\left(\omega_{k}-\epsilon_{k}\right)}{\omega_{k}\epsilon_{k}^{2}\left(\omega_{k}+\epsilon_{k}\right)^{2}\left(\omega_{k}-\epsilon_{k}\right)^{2}},\\
    &\approx\int \frac{d^{3}k}{\left(2\pi\right)^{3}} \, \left(\frac{-2}{\epsilon_{k}M^{4}}+\frac{2}{\omega_{k}M^{4}}\right).
    \end{aligned}
\end{equation}
To the order $O(\frac{1}{M^{2}})$, we only need to keep $\int \frac{d^{3}k}{\left(2\pi\right)^{3}} \frac{-2}{\omega_{k}M^{4}} $. In total we have the contribution from Figure \ref{fig:ch33d} to be
\begin{equation}\label{eq:x}
    \begin{aligned} &\frac{\lambda_{1}^{2}\lambda_{0}}{16} \int d^{3}x\, \phi(x)^{4} \int \frac{d^{3}k}{\left(2\pi\right)^{3}} \left(\frac{2}{\omega_{k}M^{4}}+\frac{1}{\epsilon_{k}^{3}M^{2}}\right),\\
    & =-\frac{\lambda_{1}^{2}\lambda_{0}}{64\pi^{2}M^{2}}\int d^{3}x\, \phi(x)^{4} \left(\left(\frac{1}{\overline{\epsilon}}+1-\ln\frac{M^{2}}{\mu^{2}}\right)-\left(\frac{1}{\overline{\epsilon}}-\ln\frac{m^{2}}{\mu^{2}}\right)\right)m=,\\
    &= -\frac{3\lambda_{0}\lambda_{1}^{2}}{8\pi^{2}M^{2}}\left(1-\ln\frac{M^{2}}{\mu^{2}}+\ln\frac{m^{2}}{\mu^{2}}\right)\int d^{3}x \, \frac{\phi(x)^{4}}{4!}.
    \end{aligned}
\end{equation}
\indent Taking $\mu \approx M$ and summing the contributions from the four diagrams together, we get the final result of four point functions at one loop level, up to order $O(\frac{1}{M^{2}})$:
\begin{equation}
    \begin{aligned} &-\frac{3\lambda_{0}^{2}}{32\pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln\frac{m^{2}}{M^{2}}\right)\int d^{3}x \, \frac{\phi(x)^{4}}{4!}-\frac{3\lambda_{2}^{2}}{32\pi^{2}}\frac{1}{\overline{\epsilon}}\int d^{3}x \, \frac{\phi(x)^{4}}{4!}\\
    &+\frac{3\lambda_{1}^{2}\lambda_{0}}{16\pi^{2}M^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln\frac{m^{2}}{M^{2}}\right)\int d^{3}x \, \frac{\phi(x)^{4}}{4!}-\frac{3\lambda_{1}^{2}\lambda_{0}}{8\pi^{2}M^{2}}\left(1+\ln\frac{m^{2}}{M^{2}}\right)\int d^{3}x \, \frac{\phi(x)^{4}}{4!}
    \end{aligned}
\end{equation}
\subsection{Renormlization}
\label{sec:ch33}
We argued in section \ref{subsec:ch23} that the UV divergences in the calculation of $H_{decoupled}$ contain information regarding the renormalization of $H_{1}$. Let's first write $H_{1}$ as
\begin{equation}
    \begin{aligned} H_{1}=\int d^{3}x\,\frac{1}{2}(\partial \phi_{bare}(x))^{2}+\frac{1}{2}m_{bare}^{2}\phi_{bare}^{2}(x)+\frac{\lambda_{0}^{bare}}{4 !}\phi_{bare}^{4}(x),
    \end{aligned}
\end{equation}
and then introduce the renormalization Z factor such that
\begin{subequations}\label{eq:y}
\begin{align}
\label{eq:y:1}
& \phi_{bare}=\sqrt{Z_{\phi}}\phi,\\
\label{eq:y:2}
&m_{bare}=\sqrt{Z_{m}}m,\\
\label{eq:y:3}
&\lambda_{0}^{bare}=Z_{\lambda_{0}}\lambda_{0}.
\end{align}
\end{subequations}
Expanding these Z factors in terms of $\frac{1}{\overline{\epsilon}}$, we have
\begin{subequations}\label{eq:y}
\begin{align}
\label{eq:y:1}
&Z_{\phi}=1+\delta^{1}_{\phi}(\frac{1}{\overline{\epsilon}})+O(\frac{1}{\overline{\epsilon}^{2}}),\\
\label{eq:y:2}
&Z_{m}=1+\delta^{1}_{m}(\frac{1}{\overline{\epsilon}})+O(\frac{1}{\overline{\epsilon}^{2}}),\\
\label{eq:y:3}
&Z_{\lambda_{0}}=1+\delta^{1}_{\lambda_{0}}(\frac{1}{\overline{\epsilon}})+O(\frac{1}{\overline{\epsilon}^{2}}).
\end{align}
\end{subequations}
Implementing these expansion, we can rewrite $H_{1}$ as
\begin{equation}
    \begin{aligned}
    H_{1}=&\int d^{3}x\, \frac{1}{2}(\partial\phi(x))^{2}+\frac{1}{2}m^{2}\phi^{2}(x)+\frac{\lambda_{0}}{4 !}\phi^{2}(x)\\
    & \frac{1}{2}\delta_{\phi}^{1}(\partial\phi(x))^{2}+\frac{1}{2}(\delta_{\phi}^{1}+\delta_{m}^{1})m^{2}\phi^{2}(x)+\frac{\lambda_{0}}{4 !}(2\delta_{\phi}^{1}+\delta_{\lambda_{0}}^{1})\phi^{4}(x)+O(\frac{1}{\overline{\epsilon}^{2}}).
    \end{aligned}
\end{equation}
Using $\overline{MS}$ scheme, we can cancel the UV divergences in $H_{decoupled}$ by counterterms in $H_{1}$. From two point calculation in section \ref{subsubsec:ch321}, we have UV divergence:
\begin{equation}
    \begin{aligned} \left(-\frac{\lambda_{0}m^{2}}{32\pi^{2}}-\frac{\lambda_{2}M^{2}}{32\pi^{2}}+\frac{\lambda_{1}^{2}m^{2}}{32\pi^{2}M^{2}}-\frac{\lambda_{1}^{2}}{16\pi^{2}}\right)\frac{1}{\overline{\epsilon}}\int d^{3}x\, \frac{\phi^{2}(x)}{2}.
    \end{aligned}
\end{equation}
From four point calculation in section \ref{subsubsec:ch322}, we have UV divergence:
\begin{equation}
    \begin{aligned}
    \left(-\frac{3\lambda_{0}^{2}}{32\pi^{2}}-\frac{3\lambda_{2}^{2}}{32\pi^{2}}+\frac{3\lambda_{1}^{2}\lambda_{0}}{16\pi^{2}M^{2}}\right)\frac{1}{\overline{\epsilon}}\int d^{3}x\,\frac{\phi^{4}(x)}{4 !}.
    \end{aligned}
\end{equation}
Since, there's no term proportional to the momentum, we know $\delta_{\phi}^{1} = 0$. Then we can use the following renormalization conditions:
\begin{subequations}
\begin{align}
&\left(\delta_{m}^{1}m^{2}+\left(-\frac{\lambda_{0}m^{2}}{32\pi^{2}}-\frac{\lambda_{2}M^{2}}{32\pi^{2}}+\frac{\lambda_{1}^{2}m^{2}}{32\pi^{2}M^{2}}-\frac{\lambda_{1}^{2}}{16\pi^{2}}\right)\frac{1}{\overline{\epsilon}}\right)\int d^{3}x\, \frac{\phi^{2}(x)}{2}=0,\\
&\left(\delta_{\lambda_{0}}^{1}\lambda_{0}+\left(-\frac{3\lambda_{0}^{2}}{32\pi^{2}}-\frac{3\lambda_{2}^{2}}{32\pi^{2}}+\frac{3\lambda_{1}^{2}\lambda_{0}}{16\pi^{2}M^{2}}\right)\frac{1}{\overline{\epsilon}}\right)\int d^{3}x\, \frac{\phi^{4}(x)}{4 !}=0,
\end{align}
\end{subequations}
to obtain
\begin{subequations}
\begin{align}
    &\delta_{\phi}^{1}=0,\\
    &\delta_{m}^{1}=\frac{1}{m^{2}}\left(\frac{\lambda_{0}m^{2}}{32\pi^{2}}+\frac{\lambda_{2}M^{2}}{32\pi^{2}}-\frac{\lambda_{1}^{2}m^{2}}{32\pi^{2}M^{2}}+\frac{\lambda_{1}^{2}}{16\pi^{2}}\right)\frac{1}{\overline{\epsilon}},\\
    &\delta_{\lambda_{0}}^{1}=\frac{1}{\lambda_{0}}\left(\frac{3\lambda_{0}^{2}}{32\pi^{2}}+\frac{3\lambda_{2}^{2}}{32\pi^{2}}-\frac{3\lambda_{1}^{2}\lambda_{0}}{16\pi^{2}M^{2}}\right)\frac{1}{\overline{\epsilon}},
\end{align}
\end{subequations}
which agree with the results from the traditional renormalization in a Lagrangian framework.

==> EFT/EFT.tex <==
\section{Construction of Effective Field Theories}
\label{sec:EFT}
In this chapter we will use the results from chapter \ref{sec:Calc} to construct the effective field theory up to order $O(\frac{1}{M^{2}})$, and show the extra finite terms in $H_{decoupled}$ are indeed canceled during matching. \\
\begin{figure}[t]
\centering 
\subfigure[]{\includegraphics[width=.25\textwidth]{Figures/4pt1.png}\label{fig:ch41a}}
\hfill
\subfigure[]{\includegraphics[width=.35\textwidth]{Figures/4pt2.png}\label{fig:ch41b}}
\hfill
\caption{\label{fig:i} Tree level contributions in $H_{decoupled}$.}
\end{figure}
\indent In $H_{decoupled}$, at tree level up to order $O(\frac{1}{M^{2}})$, we have $(\lambda_{0}-\frac{3\lambda_{1}}{M^{2}})\int d^{3}x \, \frac{\phi^{4}(x)}{4 !}$ that corresponds to Figure \ref{fig:ch41a} and Figure \ref{fig:ch41b}. First, matching the decoupled Hamiltonian at tree level onto the low energy subspace, we have
\begin{equation}
    \begin{aligned} H_{eff}^{tree} = \int d^{3}x\, \frac{1}{2}(\partial\phi(x))^{2}+\frac{1}{2}m^{2}\phi^{2}(x)+(\lambda_{0}-\frac{3\lambda_{1}}{M^{2}})\frac{\phi^{4}(x)}{4 !}+O(\frac{1}{M^{4}}).
    \end{aligned}
\end{equation}
As we claimed in section \ref{subsec:ch23}, to proceed to one loop level, we need to decouple and renormalize $H_{eff}^{tree}$ as well. To do this, we first change the low frequency modes $\phi$'s in $H_{eff}^{tree}$ back to the full light field $\Phi_{L}$. Then we can follow the similar process to decouple the high frequency and low frequency modes by unitary transformations.
\begin{equation}
    \begin{aligned} H_{decoupled}^{'}=\bra{0_{high}}\omega^{'\dagger}H_{eff}^{tree}\omega^{'}\ket{0_{high}},
    \end{aligned}
\end{equation}
where $H_{decoupled}^{'}$ is the decoupled Hamiltonian corresponding to $H_{eff}^{tree}$ and $\omega^{'}$ is the corresponding unitary transformation.\\
\begin{figure}[t]
\centering 
\includegraphics[width=.35\textwidth]{Figures/A.png}
\caption{\label{fig:ch42} One loop two point function contribution in $H_{decoupled}^{'}$}
\end{figure}
\indent First, we have a contribution from a two point function shown in Figure \ref{fig:ch42}. The calculation here is similar to the calculation of Figure \ref{fig:ch31a}, and we only need to substitute $\lambda_{0}$ with $\lambda_{0}-\frac{3\lambda_{1}^{2}}{M^{2}}$. Therefore, the result is 
\begin{equation}
    \begin{aligned} -\frac{m^{2}}{32\pi^{2}}(\lambda_{0}-\frac{3\lambda_{1}^{2}}{M^{2}})(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{\mu^{2}}}+1)\int d^{3}x \, \frac{\phi^{2}(x)}{2}+\frac{\lambda_{0}-\frac{3\lambda_{1}^{2}}{M^{2}}}{4}C\int d^{3}x\, \frac{\phi^{2}(x)}{2},
    \end{aligned}
\end{equation}
where $C=-\int_{k<M}\frac{d^{3}k}{(2\pi)^{3}}\,\frac{1}{\sqrt{k^{2}+m^{2}}}$ is the same as in section \ref{subsubsec:ch321}. Then we do the renormalization in $\overline{MS}$ scheme to cancel out the divergent part and take $\mu \approx M$. The finite terms left are
\begin{equation}
    \begin{aligned} -\frac{m^{2}}{32\pi^{2}}(\lambda_{0}-\frac{3\lambda_{1}^{2}}{M^{2}})(-\ln{\frac{m^{2}}{M^{2}}}+1)\int d^{3}x \, \frac{\phi^{2}(x)}{2}+\frac{\lambda_{0}-\frac{3\lambda_{1}^{2}}{M^{2}}}{4}C\int d^{3}x\, \frac{\phi^{2}(x)}{2}.
    \end{aligned}
\end{equation}
To do the matching, we use the finite terms in eq.(3.33) from section \ref{subsubsec:ch321} to subtract eq.(4.4) to get the two point interactions to be added in $H_{eff}^{one\,loop}$:
\begin{equation}
    \left(-\frac{\lambda_{2}M^{2}}{32\pi^{2}}-\frac{\lambda_{1}^{2}}{16\pi^{2}}-\frac{\lambda_{1}^{2}m^{2}}{16\pi^{2}M^{2}}\right) \int d^{3}x \, \frac{\phi^{2}(x)}{2}-\frac{\lambda_{1}^{2}}{32\pi^{2}M^{2}}\int d^{3}x\, \frac{1}{2}(\partial\phi(x))^{2}.
\end{equation}
As we expect the extra finite terms are all canceled out along with the large log terms during matching and will not appear in the effective Hamiltonian.\\
\begin{figure}[t]
\centering 
\includegraphics[width=.35\textwidth]{Figures/4a.png}
\caption{\label{fig:ch43} One loop four point function contribution in $H_{decoupled}^{'}$}
\end{figure}
\indent We can then consider the contribution from the four point function shown in Figure \ref{fig:ch43}. Again the calculation is similar to the one of Figure \ref{fig:ch33a}, and we only need to substitute $\lambda_{0}$ with $\lambda_{0}-\frac{3\lambda_{1}^{2}}{M^{2}}$. Hence, we have
\begin{equation}
    \begin{aligned} -\frac{3\left(\lambda_{0}-\frac{3\lambda_{1}^{2}}{M^{2}}\right)^{2}}{32\pi^{2}}\left(\frac{1}{\overline{\epsilon}}-\ln{\frac{m^{2}}{M^{2}}}\right)\int d^{3}x\, \frac{\phi^{4}(x)}{4 !}.
    \end{aligned}
\end{equation}
After renormalization, up to order $O(\frac{1}{M^{2}})$, we are left with
\begin{equation}
    \begin{aligned} \left(\frac{3\lambda_{0}^{2}}{32\pi^{2}}-\frac{9\lambda_{1}^{2}\lambda_{0}}{16\pi^{2}M^{2}}\right)\ln{\frac{m^{2}}{M^{2}}}\int d^{3}x\,\frac{\phi^{4}(x)}{4 !}.
    \end{aligned}
\end{equation}
Using the finite terms in eq.(3.55) from section \ref{subsubsec:ch322} to subtract eq.(4.7), we get the four point interactions to be added in $H_{eff}^{one loop}$ as
\begin{equation}
    -\frac{3\lambda_{0}\lambda_{1}^{2}}{8\pi^{2}M^{2}}\int d^{3}x \, \frac{\phi^{4}(x)}{4 !}.
\end{equation}
Large log terms are again canceled during matching as we expect. In conclusion, up to order $O(\frac{1}{M^{2}})$, the effective Hamiltonian at one loop level so constructed based on our theory is
\begin{equation}
    \begin{aligned} H_{eff}^{one loop}=&\int d^{3}x\, \frac{1}{2}(\partial\phi(x))^{2}+\frac{1}{2}m^{2}\phi^{2}(x)-\left(\frac{\lambda_{2}M^{2}}{32\pi^{2}}+\frac{\lambda_{1}^{2}}{16\pi^{2}}(1+\frac{m^{2}}{M^{2}})\right)\frac{\phi^{2}(x)}{2}\\
    &+\left(\lambda_{0}-\frac{3\lambda_{1}^{2}}{M^{2}}-\frac{3\lambda_{0}\lambda_{1}^{2}}{8\pi^{2}M^{2}}\right)\frac{\phi^{4}(x)}{4 !}-\frac{\lambda_{1}^{2}}{32\pi^{2}M^{2}} \frac{1}{2}(\partial\phi(x))^{2}.
    \end{aligned}
\end{equation}
